An HCI-Centric Survey and Taxonomy of Human-Generative-AI Interactions

Generative AI (GenAI) has shown remarkable capabilities in generating diverse and realistic content across different formats like images, videos, and text. In Generative AI, human involvement is essential, thus HCI literature has investigated how to effectively create collaborations between humans and GenAI systems. However, the current literature lacks a comprehensive framework to better understand Human-GenAI Interactions, as the holistic aspects of human-centered GenAI systems are rarely analyzed systematically. In this paper, we present a survey of 291 papers, providing a novel taxonomy and analysis of Human-GenAI Interactions from both human and Gen-AI perspectives. The dimensions of design space include 1) Purposes of Using Generative AI, 2) Feedback from Models to Users, 3) Control from Users to Models, 4) Levels of Engagement, 5) Application Domains, and 6) Evaluation Strategies. Our work is also timely at the current development stage of GenAI, where the Human-GenAI interaction design is of paramount importance. We also highlight challenges and opportunities to guide the design of Gen-AI systems and interactions towards the future design of human-centered Generative AI applications.

==> texes/archived/3-Input-Output.tex <==
\section{Input and Ouput}

In this section, we talk about the fundamental elements from the AI side in the context of human-GenAI interactions - the input and output of the model.
The definition of input and output in our scope lies in the context of a GenAI model rather than an interactive GenAI system, i.e., the core data perceived by the model to perform its generative task rather than the interactions or instructions to the system involving the broader user experience and how users interact with the system.

To identify the capabilities of GenAI in various contexts and discuss how the capabilities are to be utilized by human users accordingly, we propose to categorize the GenAI systems by (1) \textbf{input and output modalities}, (2) \textbf{input initialization}, and (3) \textbf{output synchronization}.
We first reveal the different modality combinations and the possible applications they can be utilized in.
Then we discover two initialization methodologies, namely \textit{user-initialization} and \textit{system-initialization}.
Finally, we discuss three synchronization methodologies, \textit{preliminary}, \textit{real-time}, and \textit{delayed}.


%\subsection{Dimension-1 Modalities}
\textit{\textbf{Dimension-1 Modalities:}}
GenAI is capable of generating content of various forms given specific inputs and conditions.
We will start with the \textbf{input modalities} and expand on the possible output modalities.

% start with input modalities and describe the possible pairs (symmetric)
% modality pairs -> quantities pairs -> different applications
% text to text -> single to single -> translation

% text to text
% text to image
% text to code
% text to data
% text to audio
\textit{Text:} Natural language information in the text constitutes the most common input modality for GenAI models.
Text can be used as the input to obtain textual output, to accomplish the tasks of translation~\cite{arakawa2022vocabencounter}, co-writing~\cite{mirowski2023co, petridis2023anglekindling, yuan2022wordcraft, swanson2021story}, or conversation~\cite{zamfirescu2023herding, valencia2023less}. Text can also be used as guidance for GenAI models to create one~\cite{} or multiple~\cite{} image depicting the text content.
Some models are capable of summarizing the information from multiple text inputs and visualizing them in a single imagery output~\cite{}.
Text with natural language information is an intuitive way to convey the requirement for a process or an algorithm.
Some GenAI models utilize this intuition and enable text-to-code generation~\cite{}.
Alternatively, the contained information in natural language text can be exploited to depict a sentimental sound effect~\cite{}, a contextual background sound~\cite{}, or a piece of artistic music~\cite{}.
Moreover, GenAI is also capable of generating numerical data (e.g., robotic control sequence~\cite{} and social computing~\cite{}), or textual data (e.g., synthetic HCI user study~\cite{} and natural language instructions to robot~\cite{}) from text inputs.

% image to image
% image to data
% image to 3D model
% image to audio
\textit{Image:} Image is a powerful input modality for GenAI models, for its rich information from visual contents and representations. 
This modality is particularly valuable in fields such as art, design, entertainment, virtual reality, fashion, and beyond.
Image-to-Image GenAI is the most common deployment of modality combination with images as inputs, fulfilling various tasks such as style transferring from image(s) to image(s)~\cite{}, image editing by reference~\cite{}, co-creation of artistic paintings~\cite{}, and image synthesis~\cite{}.
Besides, some GenAI models~\cite{} enable combinations of elements from multiple imagery inputs and apply them to the output(s), utilized in the applications like guided gallery generation~\cite{}, design ideation~\cite{}.
The rich information contained in images can be processed and guide the generation of data in other forms.
Given images as inputs, models can summarize the content~\cite{}, style~\cite{}, or even sentiment~\cite{} in the image and express by outputting text.
Images can also be used as semantic guidance for generating 3D models~\cite{}, audio~\cite{}.

% video(sequence of image) to text
\textit{Video:} Video can be seen as a time series of static images, enriching the information with a time dimension.
Based on the input video, GenAI models are capable of extracting various types of numerical data and accomplishing generating tasks based on numerical data, e.g., similar camera layouts from the video~\cite{}, segmentations of the video~\cite{}, textual content description~\cite{}, etc.

% sketch to image
% sketch to text
% sketch to 3D model
\textit{Sketch:} Sketch is also a special type of imagery input, as simple or detailed drawings that capture the basic structure or concept of an object, scene, or idea.
Using lines and shapes to convey information without the need for intricate details, sketches can be used as blueprints for GenAI to generate images enriched with textures and colors~\cite{}.
Moreover, GenAI is capable of comprehending the human intuition behind the visual representation of sketches, generating a corresponding description in natural language~\cite{}, co-creating with humans on the sketches~\cite{}, or uplifting the 2D representations into 3D space~\cite{}.

% audio to audio
% audio to text
\textit{Audio:} Audio is another powerful modality that can serve as input for generative AI systems to absorb a wide range of auditory content, from natural language speaking of the human, sound effects, music, and beyond.
GenAI-based chatbots can be deployed with the ability to take auditory natural language input and generate textual response~\cite{}.
This ability to comprehend and convert auditory features is also taken advantage of in applications such as music creation based on reference~\cite{} and music visualization~\cite{}.

% code to text
% code to code
\textit{Code:} In the context of programming, code can be used as the input for GenAI models for code comprehension~\cite{}, code generation or optimization~\cite{}, textual comment generation~\cite{}, code presentation in text and figures~\cite{}, etc.

\textit{Data:} All modalities of input can be fundamentally regarded as numerical data in the computer science and engineering realm.
In addition to the aforementioned modalities that contain high-level information that can be directly perceived by humans (e.g. image, audio, and sketch), we identify the numerical data otherwise conveying information and being used as inputs to GenAI.
For instance, brain signals can be used to guide the generation of images due to the preference information contained~\cite{}.
Among all selected research, we identified similar applications such as hair shape to hair 3D model generation~\cite{lyu2020real, shen2020deepsketchhair}, interaction logs to UI design~\cite{lee2019smartphone, he2022iplan,hu2020graph2plan, jing2023layout}, general numerical data to graphical visualization~\cite{zehrung2021vis, wang2023slide4n}, font adaptation via GenAI~\cite{aksan2018deepwriting, kadner2021adaptifont, aksan2021generative}, and gesture-based interaction design~\cite{}.
This capability of understanding numerical data has also enabled specific applications targeting the research in GenAI itself.
In~\cite{kahng2018gan}, user-modified data is used as the input to the GenAI generating visualizations of the intermediate layers for interpretability.
In addition to specified data input, GenAI is also capable of taking randomly initialized dummy data and outputting other modalities (3D models~\cite{}, audio~\cite{}, images~\cite{}, etc.)
% data to data
% data to 3D
% data to image
% data to text
% data to sketch

% font to font
% gesture to gesture

% dummy to 3D model
% dummy to audio
% dummy to data
% dummy to image


\textbf{\textit{Dimension-2 Input Initialization}}
This category differentiates between models whose initial input comes from the users and those from the systems.

\textit{User-Initialized:} In this approach, the initial input for generating content comes directly from the user.
This method of input initialization is usually required in systems where the output is heavily dependent on the input, semantically or substantively.
For example, text-based conversational GenAI~\cite{} requires the users to input textual dialogues to generate textual responses, the topic and form of which are related to the users' input.
Similarly, image-based GenAI requires the users to provide either textual descriptions of the expected images~\cite{} or images~\cite{} or sketches~\cite{} as a reference to generate the expected images.
In similar cases like music creation~\cite{}, literature writing~\cite{}, and visual design~\cite{}, the user's input guides the direction of the generated content.

\textit{system-initialized:} In this case, the generative AI model starts generating content without any specific external input.
This could be through utilizing pre-trained patterns, internal algorithms, or some combination of initial states or conditions within the model itself.
The initial generated content is not directly guided by a user's input, and the model operates more autonomously.
With this autonomy, this method of input initialization can benefit (1) GenAI systems with non-expert~\cite{louie2020novice, kadner2021adaptifont, suh2021ai} users who do not possess knowledge of proper input, (2) systems that passively assist the users~\cite{arakawa2022vocabencounter,kadner2021adaptifont}, or (3) systems that help the users with ideation within a specific domain through vast collections of examples~\cite{ko2022we, volz2018evolving, evirgen2023ganravel,padiyath2021desainer}

Besides, we identify systems that combine both initialization methods to enable both guided generation and exploration in variations~\cite{}.


\textit{\textbf{Dimension-3 Output Synchronization}}
GenAI systems also utilize different output synchronization strategies.
We identify three strategies based on the output timing with respect to the user interaction timing.

\textit{Preliminary:}
This category describes a GenAI system with output prior to the user interaction.
The preliminary output strategy is usually utilized in the GenAI systems where users absorb the AI-generated content~\cite{arakawa2022vocabencounter} passively or as is~\cite{jo2023understanding, wang2021soloist}.
Another scenario with preliminary output is the human-GenAI collaboration tasks where GenAI takes the first move to inspire~\cite{lee2022promptiverse} or motivate~\cite{arakawa2023catalyst} the human.

\textit{Real-time:}
Real-time output is generated concurrently with human interaction with the GenAI systems.
This strategy benefits the systems with the requirement of immediate responses such as in writing suggestions~\cite{} and auto completion~\cite{}.
Moreover, real-time output is preferred when the systems consist of interaction modalities that tweak the direction, attributes, or details of the generated content.
In these systems, users expect real-time feedback generated when they are interacting.
For example, in GAN-based image generation applications~\cite{dang2022ganslider, xu2021gan, evirgen2023ganravel}, when a user is dragging a slider controlling the direction of the GAN models, the visualization of the generated images is expected to be dynamic and aligned with the slider movement.
This advantage of real-time feedback can be identified through other collaborative applications such as webtoon sketch creation~\cite{}, co-writing~\cite{}, and programming assistance~\cite{}.

\textit{Delayed}
A delayed output is generated after an explicit mark of the end of the users' interaction, e.g., hitting enter when chatting with a chatbot~\cite{}, clicking on a button to input a set of parameters~\cite{}, or evaluating and confirming by previews of the final output~\cite{}.
This strategy is common in most human-GenAI interactive applications that require descriptions of human expectations of the output, such as fashion design containing multiple layers~\cite{}, artistic image generation considering multiple attributes~\cite{}, style merging requiring multiple inputs~\cite{}, etc.
When there are multiple elements to be considered by the humans in the loop, the delayed output prioritizes users' decision-making on the final output.
Some interaction techniques require delayed output by nature.
For example, interaction with a chatbot requires input and output on a conversational basis which goes one by one.
Another example is substituting the input with a new instance~\cite{}, where models are anticipated to wait until users' decision on the new input.
Nevertheless, the computation cost is a major reason for some applications resorting to delayed output.
Although from a design perspective, real-time output is preferred for the reasons aforementioned, subject to the model size and constraints on the computational power, most image-based GenAI systems resort to delayed output for consistent user interactions~\cite{}.
%Enhancing User Experience: Understanding how humans and AI can synchronize their actions leads to more intuitive and engaging user experiences. For gaming, creative tools, or virtual assistants, this can mean more natural interactions that feel fluid and responsive.
%Facilitating Collaboration: In co-creative endeavors, effective synchronization enables humans and AI to work together seamlessly. Researching this area helps to design systems that can truly augment human creativity and productivity.

%Personalization and Adaptation: Investigating how AI can adapt to individual users through synchronization leads to more personalized interactions. This includes AI that learns and adjusts to a user's preferences, habits, and nuances.
% output time to the interaction time
% prior to interaction: preliminary
% during the interaction: real-time
% after the interaction: delayed

==> texes/archived/4-Control.tex <==
\section{Control}
This section discusses how humans interact with GenAI and with what specific aspects of the GenAI model users can interact.
To this end, this section delves into the interaction modalities and techniques employed to control the AI's output, thus facilitating effective communication of human intent to the GenAI model.   


\textit{\textbf{Dimension-1 Interaction Modalities:}}
This section focuses on how to interact with the Generative AI model. We further elaborate on the different ways through which humans can interact with GenAI. It explores the various interaction modalities and methods of communication that allow users to control GenAI systems effectively. 

\textit{Widget}
The widget allows users to interact with the GenAI model system. Interacting with the widget triggers and actions.   

\textit{Controller} controller are used to control GenAI system input-output~\cite{xu2021gan}. 

\textit{Drawing and Highlighting}
Drawing and highlighting includes making sketches\cite{twomey2022three, chung2022talebrush}, Drawings~\cite{naritomi2018foodchangelens} and highlighting input~\cite{dang2022beyond, evirgen2022ganzilla} on the input or output generated from GenAI system. Some of the examples are human sketch\cite{wu2023styleme, zhao2018compensation}, terrain~\cite{guerin2017interactive}, floorplan layout~\cite{wang2021actfloor}. It also includes masking and making drawings on a portion of the image~\cite{evirgen2023ganravel, evirgen2022ganzilla, 10.1145/3306346.3323023} and selecting (highlighting) a text~\cite{dang2022beyond, fu2023comparing} 

\textit{Text}
Text control is easily accessible and does not require specialized expertise and complex interactions. Users interact with GenAI systems by providing their query\cite{valencia2023less}, half knowledge~\cite{linzbach2023decoding}, and intention~\cite{zamfirescu2023herding}. Users can control using a word~\cite{liu2022opal}, sentences~\cite{fu2023comparing}, and paragraph\cite{chung2022talebrush}. Through the textual instructions, users can attain results that align with their requirements\cite{cheng2020sequential} or signal the necessity for improvements in the GenAI system's output\cite{lanzi2023chatgpt}.   

\textit{Brain Control} Brian control refers to the direct interaction between the human brain and GenAI systems. Brain signals provide human judgments and preferences without physical activity~\cite{de2020brain}. Brain responses are recorded via electroencephalography(EEG) and then used to interact with GenAI system~\cite{de2020brain, kangassalo2020neuroadaptive, spape2021brain, davis2022brain}. Brain-using signals allow users to convey their intentions to the GenAI system which generates content based on their preferences\cite{kangassalo2020neuroadaptive, spape2021brain}. It also provides users freedom to interpret and modify the outcomes from the GenAI system~\cite{davis2022brain}.   

\textit{Gestures}
Gesture interaction with GenAI systems encompasses the utilization of physical gestures and movements as a means of engaging with the system\cite{chung2021gestural}. These gestures can range from hand movements to sketching lines~\cite{chung2021gestural, chu2023wordgesture} by hand which are used to control and communicate with the AI. 

\textit{Voice}
Human voice commands offer a dynamic approach to manipulating and directing the outcomes of GenAI models. Through vocal prompts, users can effectively steer the generated output~\cite{liu2023wants}, leveraging their spoken instructions to guide the GenAI output. This innovative interaction method harnesses the potential of natural language and empowers users to shape the GenAI output in a more personalized[] and intuitive manner \cite{liu2023wants}.

\textit{\textbf{Dimension-2 Controlling the output}}
This section covers what part of GenAI with which humans are interacting to control the output. We categorize this purpose into two categories mainly. Firstly internal control focuses on humans modifying the GenAI model itself and secondly, external control structures their input to get specific output.  

\textit{Latent Space}
From a user point of view, latent space is the way by which the system can capture essential characteristics of user preferences~\cite{guo2021vinci} and behavior\cite{}. In most cases, users may not directly manipulate the latent space but their actions such as clicking a button~\cite{evirgen2023ganravel}, moving sliders~\cite{ko2022we,dang2022ganslider} and similar can produce the data which in turn affects the latent space. Latent space representation gives users the freedom to visualize~\cite{kahng2018gan}, explore~\cite{davis2023fashioning} and transform~\cite{mozaffari2022ganspiration} the latent space to get the desired output. Latent space allows users to potentially influence the types~\cite{jing2023layout, yuan2022wordcraft}, quantities\cite{zhang2021method}, and levels of variability\cite{evirgen2023ganravel} present in the system's outputs.  

\textit{Parameters} 
Parameters are internal variables such as weights and biases that defines models behavior and makes predictions. It allows the system to become adaptive and personalize the system for each individual user's\cite{spape2021brain}. The parameters can be changed by Fine-tuning the GenAI model to make it more suitable for specific tasks\cite{spape2021brain}.      


\textit{Hyperparameters}
These GenAI model parameters allow users to control the creativity(randomness) in the output generated from the model\cite{leinonen2023using}. During the development stage of the system, random initialization and a number of iterations for optimization step~\cite{liu2022design} can be used to control the degree of randomness. Another user-controlled hyperparameter is the \textit{temperature} which is used to control sampling distribution for the output. A higher temperature setting produces more surprising (high variations) rather creative and novel outputs while the lower setting generates similar outcomes closely to existing patterns~\cite{louie2020novice, leinonen2023using}.  
Hyperparameters can be changed by the end-user using tools that allow changing values such as a widget(sliders) or text editor\cite{louie2020novice}. 

\textit{Prompts}
Prompts refer to the specific input (i.e. image\cite{wu2023styleme}, text~\cite{jiang2022discovering}, code\cite{leinonen2023comparing}, music~\cite{frid2020music}) the user provides to instruct the model about the information or task. The quality~\cite{liu2022design} and relevance\cite{lee2022promptiverse} of the input influence the output generated from GenAI systems. Prompting varies depending on the nature of the task~\cite{yang2023dual}, level of model understanding~\cite{sanchez2023examining}, and context of interaction~\cite{jiang2022discovering}. Prompts guide the model to generate the output aligned with the user's underlying context~\cite{wu2022promptchainer} and intent. Prompts additionally serve as a means for users to prototype novel functionalities within Generation-AI models, enabling the exploration and experimentation of new tasks. This is achieved through the formulation and testing of diverse prompts, which act as experimental inputs to gauge the model's capabilities and responses in unknown tasks or domains.      

\textit{Prompt Tuning}
Prompt engineering refers to the search in the input prompts that retrieves useful information that can be interpreted and understood by the GenAI system. This includes locating, modifying, and organizing\cite{jiang2022promptmaker} input prompts to provide in-context learning of the model to provide relevant output. Prompting Engineering includes chaining of prompts~\cite{wu2022ai}, automatic prompt editing~\cite{wang2023reprompt}, providing contextual information~\cite{liu2022opal}, abstraction matching of input prompt~\cite{liu2023wants}, transforming prompt to different input modality\cite{chung2022talebrush} and manual editing of prompts~\cite{endo2022user}.      
Similar to prompting, prompt engineering also guides the content generated from the model\cite{ma2022ai} and increases the understanding of the users about the kind of input needed to use the GenAI system effectively\cite{liu2023wants}.  


\textbf{\textit{Control Iteration}}
We delve into the frequency of user interactions required to achieve the intended output. We categorize this interaction frequency into two distinct classes: "Single" and "Multiple." 

\textit{Single}
Users engage with the system in a single iteration, receiving output after providing input. Consequently, there exists no connection between the preceding user input and the current one, resulting in the absence of contextual information transfer from previous interactions. Single interactions provide quick outputs, ideal for simple queries or tasks. Some of the examples are factual information\cite{} and general queries~\cite{}. In some cases, GenAI systems also possess constraints on limiting the interaction to a single\cite{kim2022stylette, }.      

\textit{Multiple}
Users perform multiple iterations because of the difference between the user's intended output and the GenAI system output. The gap occurs because of semantic~\cite{}, cognitive\cite{}, and quality~\cite{} of the generated output. users need to engage with the system multiple times to attain the desired output. This can involve a sequence of interactions, each building upon the previous one. This iterative process allows the user to gradually build context, as the model retains information from previous interactions until the intended result is achieved. This approach provides contextually accurate\cite{} and meaningful responses\cite{}. Multiple interactions allow users to build progressive build narratives\cite{} and brainstorm ideas~\cite{}.


 

==> texes/archived/5-Feedback.tex <==
\section{Feedback}
In this section, we discuss content and information from the GenAI system are presented to the user. 

\textit{\textbf{Dimension-1 Presentation and Visualization}}
Our focus is visual representation and the specific information that is provided to the user. We delve into how data is displayed, organized, and conveyed to users in various contexts.

\textit{Canvas} A canvas refers to a space or surface where visual content, along with other elements like text, code, images, and more, can be displayed, and the user can interact with and manipulate it. Some of the examples include presentation slides~\cite{}, code cells~\cite{}, image collage~\cite{}, documents containing text with visual content {}, website~\cite{}, and drawing sheet~\cite{}.    

\textit{Text Box}
The text box displays useful information in the form of text\cite{chung2022talebrush} in the system.   

\textit{3D}
3D information includes the display of 3D CAD Models~\cite{liu20233dall, liu2023beyond} and Augmented reality\cite{zhao2018compensation}, Virtual Reality\cite{ren2023leveraging}, and real-world such as Television\cite{shirazi2021supervised}.  

\textit{graphs and charts}
Graphs and charts are used to visually convey numerical information to the user. Tabular data~\cite{liu2023wants}, music notes\cite{louie2020novice} and waveform visualization\cite{wang2021soloist} are some examples.  
It enables users to grasp complex concepts in understanding GenAI Models\cite{kahng2018gan}. Areas and layouts present numerical information, aiding designers in crafting intuitive and informative displays~\cite{jing2023layout, wang2021actfloor}. Charts help in more informed decision making such as activity learning progression in form of pie chart\cite{wang2021soloist}  

\textit{Audio}
Voice provided by the users are provided with an option to not only see but also hear their own voices, enhancing the interactive experience\cite{janssens2022cool}. Music audio~\cite{chang2018perceptual} is transmitted from audio speakers to the user's. Audio output is effortless to consume and provides user's richer and more engaging experience when combined with visuals\cite{wang2021toward}. 


\textit{\textbf{Dimension-2 Content of Feedback}}
The content focuses on the various types of data the user can see, which can be broadly categorized into three distinct groups: input from the user, intermediate results, and final output. These categories help users organize and understand the flow of information within a system.   

\textit{Input}
This category includes any data or information that the user provides to the system and system-initialized information. It's the initial information that the system uses as a starting point for its operations. Initial data such as input text\cite{strobelt2022interactive, leinonen2023using}, file or image upload\cite{}, random noise~\cite{kahng2018gan} and selections made in the input\cite{fu2023comparing} are shown to the user.   

\textit{Intermediate}
Various calculations, transformations, and operations performed by the GenAI system are shown to the user. Latent space\cite{dang2022ganslider, evirgen2023ganravel}, heatmaps\cite{kahng2018gan, wang2021actfloor} are some examples of intermediate results. 

\textit{Final Output}
The ultimate information or outcomes that the system generates are based on the user's input and the processing of intermediate results. The final output is what the user typically seeks when interacting with the system. The final output is always shown to the user. In some cases final output is shown with intermediate\cite{wu2023styleme} or input to the user~\cite{ross2021evaluating} or both together~\cite{dang2022ganslider}. 

